Proximal Gradient Algorithms under Local Lipschitz Gradient Continuity: A Convergence and Robustness Analysis of PANOC

Composite optimization offers a powerful modeling tool for a variety of applications and is often numerically solved by means of proximal gradient methods. In this paper, we consider fully nonconvex composite problems under only local Lipschitz gradient continuity for the smooth part of the objective function. We investigate an adaptive scheme for PANOC-type methods (Stella et al. in Proceedings of the IEEE 56th CDC, 1939--1944, 2017), namely accelerated linesearch algorithms requiring only the simple oracle of proximal gradient. While including the classical proximal gradient method, our theoretical results cover a broader class of algorithms and provide convergence guarantees for accelerated methods with possibly inexact computation of the proximal mapping. These findings have also significant practical impact, as they widen scope and performance of existing, and possibly future, general purpose optimization software that invoke PANOC as inner solver.

==> TeX/Tikz/counterexamplebox.tex <==
\begin{tikzpicture}
	\begin{groupplot}[
		width=.5\linewidth,
		height=.35\linewidth,
		group style={
			group size= 2 by 2,
			vertical sep=3.5em,
			horizontal sep=3.5em},
		grid=major,
		grid style={line width=.1pt, draw=gray!30},
		% major grid style={line width=.2pt,draw=gray!60},
		xmin = 1,
		xmax = 10001,
		xmode=log,
		ymode=log
		]
		
		% Iterate \bar x
		\nextgroupplot[title=Iterate \(\bar{x}^k\), title style = {inner sep=0pt,outer sep=0pt}]
		\addplot [color=origcolor, mark=\origmarker, mark options={solid, origcolor}]
		table {TeX/Tikz/Data/counterexamplebox/xbar_orig.dat};\label{plot:orig:1}
		\addplot [color=pluscolor, mark=\plusmarker, mark options={solid, pluscolor}]
		table {TeX/Tikz/Data/counterexamplebox/xbar_plus.dat};\label{plot:plus:1}
		\coordinate (top) at (rel axis cs:0,1);% coordinate at top of the first plot
		
		% Stepsize \gamma
		\nextgroupplot[title=Proximal stepsize \(\gamma_k\), ymin = 0.001, title style = {inner sep=0pt,outer sep=0pt}]
		\addplot [color=origcolor, mark=\origmarker, mark options={solid, origcolor}]
		table {TeX/Tikz/Data/counterexamplebox/gamma_orig.dat};
		\addplot [color=pluscolor, mark=\plusmarker, mark options={solid, pluscolor}]
		table {TeX/Tikz/Data/counterexamplebox/gamma_plus.dat};
		
		% FBE
		\nextgroupplot[title=FBE \(\FBE(x^k)\), title style = {inner sep=0pt,outer sep=0pt}]
		\addplot [color=origcolor, mark=\origmarker, mark options={solid, origcolor}]
		table {TeX/Tikz/Data/counterexamplebox/FBE_orig.dat};
		\addplot [color=pluscolor, mark=\plusmarker, mark options={solid, pluscolor}]
		table {TeX/Tikz/Data/counterexamplebox/FBE_plus.dat};
		
		
		% Residual (x - \bar x) / \gamma
		\nextgroupplot[title=Residual \(\|x^k-\bar x^k\|/\gamma_k\), title style = {inner sep=0pt,outer sep=0pt}]
		\addplot [color=origcolor, mark=\origmarker, mark options={solid, origcolor}]
		table {TeX/Tikz/Data/counterexamplebox/res_orig.dat};
		\addplot [color=pluscolor, mark=\plusmarker, mark options={solid, pluscolor}]
		table {TeX/Tikz/Data/counterexamplebox/res_plus.dat};
		\coordinate (bot) at (rel axis cs:1,0);% coordinate at bottom of the last plot
	\end{groupplot}
	
	% legend
	\path (top|-current bounding box.north)--
	coordinate(legendpos)
	(bot|-current bounding box.north);
	\matrix[
	matrix of nodes,
	anchor=south,
	draw,
	inner sep=0.2em,
	] at ([yshift=1ex]legendpos) {
		\ref{plot:orig:1}& PANOC &[5pt] \ref{plot:plus:1}& PANOC$^{+}$\\};
\end{tikzpicture}


==> TeX/Tikz/counterexamplebox_merit.tex <==
\begin{tikzpicture}

\begin{axis}[%
	width=.45\linewidth,
	height=.3\linewidth,
% 	width=.5\linewidth,
% 	height=.3\linewidth,
% 	at={(0,0)},
	scale only axis,
	xmin=0,
	xmax=1.2,
	xtick={0,0.25,0.5,0.75,1},
	xticklabels={0,,0.5,,1},
% 	xlabel={\(x\)},
	ymin=-0.05,
	ymax=0.2,
	ytick={0,0.05,0.1,0.15,0.2},
	yticklabels={0,,0.1,,0.2},
	grid=major,
	grid style={line width=.1pt, draw=gray!30},
	legend style={at={(0.03,0.97)}, anchor=north west, legend cell align=left, align=left, draw=white!15!black}
]
	% f
	\addplot [color=black, dotted, line width=2.0pt] table {TeX/Tikz/Data/counterexamplebox_merit/f.dat};
	\addlegendentry{\(\varphi(x)\)}
	
	% PANOC
	\addplot [color=origcolor, \origlinestyle, line width=2.0pt] table {TeX/Tikz/Data/counterexamplebox_merit/orig.dat};
	\addlegendentry{\(\def\iter{k-1}\FBE(x)\)}
	
	% PANOC+
	\addplot [color=pluscolor, \pluslinestyle, line width=2.0pt] table {TeX/Tikz/Data/counterexamplebox_merit/plus.dat};
	\addlegendentry{\(\def\iter{k}\FBE(x)\)}

\end{axis}
\end{tikzpicture}%

